The partial copula: Properties and associated dependence measures

The partial correlation coefficient is a commonly used measure to assess the conditional dependence between two random variables. We provide a thorough explanation of the partial copula, which is a natural generalization of the partial correlation coefficient, and investigate several of its properties. In addition, properties of some associated partial dependence measures are examined.

==> preamble/Commands.tex <==
%%%%% COMMANDS %%%%
%--- general commands
\newcommand{\tc}{\textcolor}
\newcommand{\approxsign}[1]{\tilde{#1}}
\newcommand{\KL}[2]{D_{KL}(#1||#2)} % KL divergence
\newcommand{\parderiv}[2]{\partial_{#2}{#1}} % partial derivative
\newcommand{\as}{a.s.} 
\newcommand{\ivb}[1]{1\!\!1_{\{#1\}}} % iversion bracket
\renewcommand{\P}{\mathbb{P}}
\newcommand{\expec}{\mathbb{E}}
\newcommand{\cov}{\mathbb{C}\text{ov}}
\newcommand{\var}{\mathbb{V}\text{ar}}
\newcommand{\E}{{\cal E}}
\newcommand{\corr}{\mathbb{C}\text{orr}}
\newcommand{\indep}{\perp\!\!\!\perp}
\renewcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\renewcommand{\indep}{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\eq}{\Leftrightarrow}
\newcommand{\imp}{\Rightarrow}
\newcommand{\std}[2]{\operatorname*{\!\!\!\!\!\!\!\!\phantom{_p}#1\phantom{_p}\!\!\!\!\!\!\!\!}_{#2}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%--- vine copula related commands
\newcommand{\SPCC}{\mathfrak} % space of simplified pcc
\newcommand{\idxset}{{\cal I}_K}
\newcommand{\parsign}[1]{#1^{\text{\tiny P}}} % partial copula
\newcommand{\pvc}[1]{#1^{\text{\tiny PVC}}} % j-th order partial copula
\newcommand{\condset}{S_{ij}} % conditioning variables
\newcommand{\sarg}[2]{S_{#1,#2}}
\newcommand{\cs}{|}
\newcommand{\ps}{;\,}
\renewcommand{\ps}{;\kern 0.08em}
%\renewcommand{\ps}{{\kern 0.06em} ;\kern 0.02em}
\renewcommand{\ps}{;}




==> preamble/autoref_setup.tex <==
%%%%%%%%%% Define commands for automatic referencing
\let\orgautoref\autoref
\providecommand{\autorefs}
         {\def\sectionautorefname{Sections}%
         \def\subsectionautorefname{Sections}%
         \def\subfigureautorefname{Figures}%
         \def\mydefautorefname{Definitions}%
         \def\myexautorefname{Examples}%
         \def\mylemautorefname{Lemmas}%
         \def\myremautorefname{Remarks}%
         \def\mytheautorefname{Theorems}%
         \orgautoref}
         \providecommand{\appref}
{\def\subsectionautorefname{Appendix}%
         \orgautoref}
\renewcommand{\autoref}
        {\def\mydefautorefname{Definition}%
         \def\figureautorefname{Figure}%
         \def\subfigureautorefname{Figure}%
         \def\sectionautorefname{Section}%
         \def\subsectionautorefname{Section}%
         \def\mypropautorefname{Property}%
         \def\mycorautorefname{Corollary}%
         \def\subtableautorefname{Table}%
         \def\tableautorefname{Table}%
         \def\myexautorefname{Example}%
         \def\mylemautorefname{Lemma}%
         \def\myremautorefname{Remark}%
         \def\mytheautorefname{Theorem}%
         \orgautoref}
\makeatletter
\let\@autoref=\autoref
\renewcommand*{\autoref}[2][]{\ifthenelse{\equal{#1}{}}{\@autoref{#2}}{\hyperref[#1]{\begin{NoHyper}\@autoref{#2}~\subref{#1}\end{NoHyper}}}\xspace}
\makeatother


==> preamble/options.tex <==

\markversion{note}
\setlength{\emergencystretch}{1em}

%%%%%%%%%% COUNTERS ETC
%\numberwithin{myprop}{section}
\numberwithin{mycor}{section}
%\numberwithin{myex}{section}
\numberwithin{mydef}{section}
\numberwithin{mylem}{section}
\numberwithin{myrem}{section}
\numberwithin{mythe}{section}
\numberwithin{equation}{section}


==> preamble/preamble.tex <==
%%%% PACKAGES %%%%
\RequirePackage{natbib}
\usepackage{amssymb}
\usepackage[bookmarksdepth,hidelinks,colorlinks=true,linkcolor=blue,citecolor=blue,filecolor=blue,urlcolor=blue]{hyperref}
\usepackage[hyperref,thmmarks]{ntheorem} % should be loaded after hyperref, there are also compatibility issues with maththools
\usepackage{graphicx}
\usepackage[labelsep=newline,font=small,labelfont=bf,singlelinecheck=false]{caption}
\usepackage{xspace}
\usepackage{ifthen}
\usepackage{mathtools}
\usepackage{subcaption}
\usepackage{multirow}
\usepackage{enumerate}
\usepackage{versions}

\usepackage[top=1in, bottom=1in, left=0.9in, right=0.9in]{geometry}
\usepackage{setspace}
\doublespacing

%%%%%%%%%% COMMANDS
\input{preamble/Commands}

%%%% OPTIONS %%%%
\input{preamble/theorem_setup}
\input{preamble/autoref_setup}
\input{preamble/options}
\captionsetup[figure]{singlelinecheck=on, labelsep=colon}

%%%% MISC %%%%
%\input{preamble/abbreviations}
\hyphenation{Ar-chi-me-dean}
\newcommand\tagging{\addtocounter{equation}{1}\tag{\theequation}}
\def\RefEqual#1{\stackrel{\text{\tiny\makebox[0pt]{#1}}}{=}}




==> preamble/theorem_setup.tex <==
\theoremstyle{break} % defines the style, 'break' inserts a line break before the %text begins
%\theorembodyfont{\slshape} % can be \rmfamily (default), \upshape, 
\theoremseparator{} % specifies the separator after the name of the theorem
\theoremprework{%
\setlength\theorempreskipamount{0.5cm}
\setlength\theorempostskipamount{0cm}
}
\newtheorem{myprop}{Property}
\newtheorem{mycor}{Corollary}
\newtheorem{mydef}{Definition}
\newtheorem{mylem}{Lemma}
\newtheorem{myrem}{Remark}
\newtheorem{mythe}{Theorem}
\theorembodyfont{\rmfamily}
\newtheorem{myex}{Example}

\theoremstyle{nonumberplain}
\theoremseparator{:}
\theoremsymbol{\ensuremath{\blacksquare}}
\theoremsymbol{}
\theoremprework{%
\setlength\theorempreskipamount{-0.5cm}
\setlength\theorempostskipamount{0cm}
}
\newtheorem{myproof}{Proof}



